When Can Proxies Improve the Sample Complexity of Preference Learning?

We address the problem of reward hacking, where maximising a proxy reward does not necessarily increase the true reward. This is a key concern for Large Language Models (LLMs), as they are often fine-tuned on human preferences that may not accurately reflect a true objective. Existing work uses various tricks such as regularisation, tweaks to the reward model, and reward hacking detectors, to limit the influence that such proxy preferences have on a model. Luckily, in many contexts such as medicine, education, and law, a sparse amount of expert data is often available. In these cases, it is often unclear whether the addition of proxy data can improve policy learning. We outline a set of sufficient conditions on proxy feedback that, if satisfied, indicate that proxy data can provably improve the sample complexity of learning the ground truth policy. These conditions can inform the data collection process for specific tasks. The result implies a parameterisation for LLMs that achieves this improved sample complexity. We detail how one can adapt existing architectures to yield this improved sample complexity.

==> figures/phi-param-vis.tex <==
\begin{figure}
    \centering
    \def\svgwidth{1\columnwidth}
    \import{figures}{phi-param-vis.pdf_tex}
    \caption{$\phi_\theta$ is implemented by first being mapped to a simplex, which is compact; this is then continuously mapped to a manifold. This ensures the boundedness of the manifold.}
\end{figure}

==> figures/pi-param-vis.tex <==
\begin{figure}
    \centering
    \def\svgwidth{1\columnwidth}
    \import{figures}{pi-parameterisation-vis.pdf_tex}
    \caption{A visualisation of the composition of $\pi^\dagger_\theta$ and $\tilde\pi_\theta$. From $\set{X}$, the yellow regions are mapped by $\tau_\theta$ to the yellow point in $\Reals[d]$, and the purple regions the purple point. $\phi_\theta$ is bijective from $\Reals[d]$ to the manifold $\tilde\pi_\theta\call{\set{X}}$ in $\set{P_X}$. Following the thick black arrows $\set{X} \to \Reals[d] \to \tilde\pi_\theta\call{\set{X}}$ gives $\tilde\pi_\theta$. Following the thick black arrows $\set{X} \to \Reals[d] \to {\color{emph} \Reals[d]} \to \tilde\pi_\theta\call{\set{X}}$ gives $\pi^\dagger_\theta$.}
\end{figure}


